Variability, periodicity and contact binaries in WISE

The time-series component of WISE is a valuable resource for the study of variable objects. We present an analysis of an all-sky sample of ~450,000 AllWISE+NEOWISE infrared light curves of likely variables identified in AllWISE. By computing periodograms of all these sources, we identify ~56,000 periodic variables. Of these, ~42,000 are short-period (P<1 day), near-contact or contact eclipsing binaries, many of which are on the main sequence. We use the periodic and aperiodic variables to test computationally inexpensive methods of periodic variable classification and identification, utilizing various measures of the probability distribution function of fluxes and of timescales of variability. The combination of variability measures from our periodogram and non-parametric analyses with infrared colors from WISE and absolute magnitudes, colors and variability amplitude from Gaia is useful for the identification and classification of periodic variables. Furthermore, we show that the effectiveness of non-parametric methods for the identification of periodic variables is comparable to that of the periodogram but at a much lower computational cost. Future surveys can utilize these methods to accelerate more traditional time-series analyses and to identify evolving sources missed by periodogram-based selections.

==> artdef.tex <==
\newcommand\aj{\sl AJ}%
          % Astronomical Journal
\newcommand\actaa{\sl Acta Astron.}%
  % Acta Astronomica
\newcommand\araa{\sl ARA\&A}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{\sl ApJ}%
          % Astrophysical Journal
\newcommand\apjl{\sl ApJ}%
          % Astrophysical Journal, Letters
\newcommand\apjs{\sl ApJS}%
          % Astrophysical Journal, Supplement
\newcommand\ao{\sl Appl.~Opt.}%
          % Applied Optics
\newcommand\apss{\sl Ap\&SS}%
          % Astrophysics and Space Science
\newcommand\aap{\sl A\&A}%
          % Astronomy and Astrophysics
\newcommand\aapr{\sl A\&A~Rev.}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{\sl A\&AS}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{\sl AZh}%
          % Astronomicheskii Zhurnal
\newcommand\baas{\sl BAAS}%
          % Bulletin of the AAS
\newcommand\caa{\sl Chinese Astron. Astrophys.}%
  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{\sl Chinese J. Astron. Astrophys.}%
  % Chinese Journal of Astronomy and Astrophysics
\newcommand\icarus{\sl Icarus}%
  % Icarus
\newcommand\jcap{\sl J. Cosmology Astropart. Phys.}%
  % Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{\sl JRASC}%
          % Journal of the RAS of Canada
\newcommand\memras{\sl MmRAS}%
          % Memoirs of the RAS
\newcommand\mnras{\sl MNRAS}%
          % Monthly Notices of the RAS
\newcommand\na{\sl New A}%
  % New Astronomy
\newcommand\nar{\sl New A Rev.}%
  % New Astronomy Review
\newcommand\pra{\sl Phys.~Rev.~A}%
          % Physical Review A: General Physics
\newcommand\prb{\sl Phys.~Rev.~B}%
          % Physical Review B: Solid State
\newcommand\prc{\sl Phys.~Rev.~C}%
          % Physical Review C
\newcommand\prd{\sl Phys.~Rev.~D}%
          % Physical Review D
\newcommand\pre{\sl Phys.~Rev.~E}%
          % Physical Review E
\newcommand\prl{\sl Phys.~Rev.~Lett.}%
          % Physical Review Letters
\newcommand\pasa{\sl PASA}%
  % Publications of the Astron. Soc. of Australia
\newcommand\pasp{\sl PASP}%
          % Publications of the ASP
\newcommand\pasj{\sl PASJ}%
          % Publications of the ASJ
\newcommand\qjras{\sl QJRAS}%
          % Quarterly Journal of the RAS
\newcommand\rmxaa{\sl Rev. Mexicana Astron. Astrofis.}%
  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{\sl S\&T}%
          % Sky and Telescope
\newcommand\solphys{\sl Sol.~Phys.}%
          % Solar Physics
\newcommand\sovast{\sl Soviet~Ast.}%
          % Soviet Astronomy
\newcommand\ssr{\sl Space~Sci.~Rev.}%
          % Space Science Reviews
\newcommand\zap{\sl ZAp}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{\sl Nature}%
          % Nature
\newcommand\iaucirc{\sl IAU~Circ.}%
          % IAU Cirulars
\newcommand\aplett{\sl Astrophys.~Lett.}%
          % Astrophysics Letters and Communications
\newcommand\apspr{\sl Astrophys.~Space~Phys.~Res.}%
          % Astrophysics Space Physics Research
\newcommand\bain{\sl Bull.~Astron.~Inst.~Netherlands}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{\sl Fund.~Cosmic~Phys.}%
          % Fundamental Cosmic Physics
\newcommand\gca{\sl Geochim.~Cosmochim.~Acta}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{\sl Geophys.~Res.~Lett.}%
          % Geophysics Research Letters
\newcommand\jcp{\sl J.~Chem.~Phys.}%
          % Journal of Chemical Physics
\newcommand\jgr{\sl J.~Geophys.~Res.}%
          % Journal of Geophysical Research
\newcommand\jqsrt{\sl J.~Quant.~Spec.~Radiat.~Transf.}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{\sl Mem.~Soc.~Astron.~Italiana}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{\sl Nucl.~Phys.~A}%
          % Nuclear Physics A
\newcommand\physrep{\sl Phys.~Rep.}%
          % Physics Reports
\newcommand\physscr{\sl Phys.~Scr}%
          % Physica Scripta
\newcommand\planss{\sl Planet.~Space~Sci.}%
          % Planetary Space Science
\newcommand\procspie{\sl Proc.~SPIE}%
          % Proceedings of the SPIE

